E2LLM: Towards Efficient LLM Serving in Heterogeneous Edge/Fog Environments

Large Language Models (LLMs) have become integral to modern applications, yet their deployment remains challenging. Beyond executing the models themselves, practical deployment must address cost efficiency, low latency, and optimal resource utilization. Conventional approaches typically assume that an entire model can be hosted on a single device, which does not hold in many real-world scenarios, particularly in Edge and Fog environments where device resources are constrained. In this paper, we introduce E2LLM, a framework designed to enable efficient LLM deployment in such resource limited settings. Rather than simply partitioning a single model across all available devices, E2LLM replicates the full model across multiple groups of devices (replicas) and applies model parallelism within each replica. Each replica is assigned a specialized role PREFILL or DECODER based on its efficiency in handling input and output tokens. This separation leverages the inherent differences between these two phases of LLM inference. To effectively organize devices, we utilize a Genetic Algorithm to form clusters that maximize system performance. Within each cluster, we apply Dynamic Programming to determine an optimal partitioning strategy that minimizes bottlenecks in model-parallel execution. Experimental results demonstrate that our approach adapts robustly to varying workloads, including scenarios with significant variation in input and output token lengths. Compared to the Splitwise baseline, E2LLM reduces average waiting time by over 50% under high-demand conditions

==> texFiles/background.tex <==


\subsection{Auto-regressive LLM Generation}
The inference process in large language models typically consists of two distinct phases: the Prefill stage and the Decoder stage. In the Prefill stage, the entire input context is processed to compute hidden states, which requires substantial computation but can be parallelized across multiple devices. Once this initialization is complete, the model enters the Decoder stage, where tokens are generated one at a time in an auto-regressive manner. This sequential dependency often becomes the main bottleneck, as each token relies on the previously generated ones. To mitigate this, modern systems employ a KV cache, which stores the key-value pairs of attention layers from previous tokens. By reusing these cached representations, the model avoids recomputing attention for past tokens, significantly reducing computation and improving decoding speed. However, when assigning roles to each replica, it is crucial to consider the KV cache transmission time between devices. The size of the KV cache grows with the sequence length and number of layers, making it extremely large. Transferring this data across devices in a distributed setup can consume significant bandwidth, leading to high transmission latency and reduced overall system efficiency. This challenge becomes even more pronounced in heterogeneous environments where network capacity is limited compared to the computational demands of large language models.

%While auto-regressive generation is the dominant approach for large language models, where tokens are produced sequentially based on previously generated tokens, recent research has explored diffusion-based methods as an alternative. Diffusion LLMs treat text generation as a denoising process, starting from a noisy representation and progressively refining it into coherent text through multiple steps. Unlike auto-regressive decoding, which is inherently sequential and latency-bound, diffusion-based generation can leverage parallelism across steps, potentially reducing inference time and enabling new optimization strategies. However, this type of generation will be let for furture work.

\subsection{Framework: llama.cpp}
llama.cpp is a lightweight framework implemented in C++, designed for efficient inference of large language models on resource-constrained devices. Its minimalistic design avoids heavy dependencies, ensuring portability and ease of deployment across platforms such as desktops, edge servers, and even mobile devices. Initially optimized for CPU execution, llama.cpp has been extended to support GPU backends like CUDA and Metal, enabling faster inference while maintaining its simplicity. Thanks to its efficiency and flexibility, llama.cpp has become the foundation for numerous chatbot applications, including LocalAI, Ollama, and LM Studio, which allow users to run conversational AI locally without relying on cloud services. 
%These applications demonstrate the practicality of llama.cpp for privacy-preserving and cost-efficient AI deployments.However, the feature of collaborating across multiple devices over a network in llama.cpp is still experimental and far from production-ready. Implementing this capability requires significant effort, particularly when integrating it with pipeline parallelism. The main challenge lies in coordinating computation stages while managing KV cache across different role, including retrieving, sending and loading cache. 

\begin{comment}
\subsection{Continuous batching}
Batching is a widely used technique to improve the efficiency of large language model inference by processing multiple requests together instead of handling them individually. When using batching, the system’s throughput increases significantly due to higher parallelism saturation, especially on hardware like NVIDIA GPUs that are optimized for large-scale parallel computation. However, batching introduces a trade-off: while throughput improves, the average time to generate a token per request becomes higher. This is because all sequences in the batch must progress in lockstep—each decoding step waits until every request in the batch completes its current token before moving to the next. 

Continuous batching is an advanced technique that improves system utilization by dynamically adding new requests to an ongoing batch as long as the batch size does not exceed the predefined maximum capacity. Unlike static batching, where all requests must arrive before processing begins, continuous batching allows inference to start immediately and incorporate additional requests on the fly. This approach significantly increases throughput and reduces idle time, especially in high-traffic scenarios, by keeping the GPU fully saturated. 

\subsection{Quality-of-Service (including SLO) in Edge/Fog Cluster Environment}
When designing and deploying LLMs in cloud environments, Quality-of-Service (QoS) metrics typically emphasize how fast the system responds to a prompt—measured as Time-To-First-Token (TTFT)—and how quickly subsequent tokens are generated, measured as Time-Per-Output-Token (TPOT). These metrics dominate because cloud servers usually have powerful hardware with abundant compute resources and high memory bandwidth, making latency the primary concern.

Contrastly, in edge and fog environments, Quality-of-Service must account for high demand under limited resources. Unlike cloud servers, edge devices have constrained compute power and memory, making it critical to define the maximum number of concurrent requests that can be processed at the same time. This limit helps minimize waiting time for new requests while ensuring that token generation speed remains acceptable for active sessions. If too many requests are admitted simultaneously, resource contention can severely degrade throughput and increase latency for all users. Therefore, adaptive admission control and scheduling policies are essential to balance fairness, responsiveness, and efficiency in edge clusters.

Studies show that people read at an average speed of about 238 words per minute \cite{brysbaert2019many}, which is roughly 4 words per second. This simple fact gives us a clear benchmark: any distributed system that delivers text-based content must ensure its performance does not slow down the reading experience. If the system introduces delays beyond this natural pace, users will notice and their experience will suffer. Therefore, we define a performance criterion based on this reading speed to guarantee smooth and uninterrupted interaction.

\end{comment}
